LibSC: Library for Scaling Correction Methods in Density Functional Theory

In recent years, a series of scaling correction (SC) methods have been developed in the Yang laboratory to reduce and eliminate the delocalization error, which is an intrinsic and systematic error existing in conventional density functional approximations (DFAs) within density functional theory (DFT). Based on extensive numerical results, the SC methods have been demonstrated to be capable of reducing the delocalization error effectively and producing accurate descriptions for many critical and challenging problems, including the fundamental gap, photoemission spectroscopy, charge transfer excitations and polarizability. In the development of SC methods, the SC methods were mainly implemented in the QM4D package that was developed in the Yang laboratory for research development. The heavy dependency on the QM4D package hinders the SC methods from access by researchers for broad applications. In this work, we developed a reliable and efficient implementation , LibSC for the global scaling correction (GSC) method and the localized orbital scaling correction (LOSC) method. LibSC will serve as a light-weight and open-source library that can be easily accessed by the quantum chemistry community. The implementation of LibSC is carefully modularized to provide the essential functionalities for conducting calculations of the SC methods. In addition, LibSC provides simple and consistent interfaces to support multiple popular programing languages, including C, C++ and Python. In addition to the development of the library, we also integrated LibSC with two popular and open-source quantum chemistry packages, the Psi4 package and the PySCF package, which provides immediate access for general users to perform calculations with SC methods.

==> my_macro.tex <==
\newcommand{\dd}{\mathop{}\!\text{d}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\asterisk}[1]{#1 \textsuperscript{*}}
\newcommand{\etal}{\textit{et al.}}
\newcommand{\schrodinger}{Schr\"{o}dinger }
\newcommand{\seeSI}[0]{Appendix}
\makeatletter
\makeatother
\newcommand{\addfootnotespace}{\vspace{2mm}}
\newcommand{\heavytoprule}{\toprule[1.5pt]}
\newcommand{\heavybottomrule}{\bottomrule[1.5pt]}
\newcommand{\loone}[0]{{\tt localization1}}
\newcommand{\lotwo}[0]{{\tt localization2}}
\newcommand{\kappaone}[0]{{\tt curvature1}}
\newcommand{\kappatwo}[0]{{\tt curvature2}}
\newcommand{\Rplus}{\protect\hspace{-.1em}\protect\raisebox{.35ex}{\smaller{\smaller\textbf{+}}}}
\newcommand{\Cpp}[0]{\mbox{C\Rplus\Rplus}}
\newcommand{\Cpponeone}[0]{\mbox{C\Rplus\Rplus11}}

